Multi-Scenario Ranking with Adaptive Feature Learning

Recently, Multi-Scenario Learning (MSL) is widely used in recommendation and retrieval systems in the industry because it facilitates transfer learning from different scenarios, mitigating data sparsity and reducing maintenance cost. These efforts produce different MSL paradigms by searching more optimal network structure, such as Auxiliary Network, Expert Network, and Multi-Tower Network. It is intuitive that different scenarios could hold their specific characteristics, activating the user's intents quite differently. In other words, different kinds of auxiliary features would bear varying importance under different scenarios. With more discriminative feature representations refined in a scenario-aware manner, better ranking performance could be easily obtained without expensive search for the optimal network structure. Unfortunately, this simple idea is mainly overlooked but much desired in real-world systems.Further analysis also validates the rationality of adaptive feature learning under a multi-scenario scheme. Moreover, our A/B test results on the Alibaba search advertising platform also demonstrate that Maria is superior in production environments.

==> algorithm_backup.tex <==


%============================================
\section{Method}\label{sec:algo}
%============================================
\begin{figure*}[htbp]
\centerline{
\includegraphics[width=1.05\textwidth]{img_new/framework_v2.pdf}}
\centering
\caption{The network architecture of our proposed \baby. The input is divided according to different feature domains. The multi-level decoupling structure is shown in (a), (b), and (c). Meanwhile, in module (a), by scaling the features and applying the Feature-level Decoupling and Interaction, the shared information and mutually exclusive data distribution deviation are better captured and distinguished respectively by the model in the training process.}
\label{fig:model}
\end{figure*}


In this section, we present the proposed \baby model in detail. As illustrated in Figure~\ref{fig:model}, the proposed \baby consists of a three-level framework: feature-level, network-level, prediction-level layers, and two main components: \textit{Scene-Awware Feature-Grained Scaling} and \textit{Feature-Level Decoupling and Interaction}. In the following, we firstly present the formal problem setting. Then, we describe these components, followed by the feature layer, network layer, prediction layer, and model optimization process.


%============================================
\subsection{Problem Formulation}\label{ssec:formulation}
%============================================

Let $\mathcal{V}=\{x_1, x_2, ..., x_M\}$ denotes the set of all items consists of products and advertisements~(Ads), $\mathcal{U}=\{u_1, u_2, ..., u_N\}$ be the set of all users, and $\{b_u\}_{M}^N$ be the behavior sequence set between these $N$ users and $M$ items. Here, for each user $u$, $b_u=[x_1, x_2, ..., x_m]$ is the sequence of her clicked items following the chronological order, and $m$ is the predefined maximum capacity. For each item $x$, it has $S$ attributes: $\mathcal{A}_x = [a_x^1, a_x^2, ..., a_x^S]$. For each user $u$, there are $L$ attributes represented by $\mathcal{A}_u = [a_u^1, a_u^2, ..., a_u^L]$ orderly. 
$N_a^u$ and $N_a^x$ denote the number of user attributes and item attributes in total respectively.
Besides, in the terms of query domain features, there are two types of queries which are mentioned above: (1)~$\mathcal{Q}=\{q_1, q_2, ..., q_K\}$ denotes the set of all query photos; 
(2)~Another queries are items, namely triggers, which is used to find similar items corresponding to it. Thus, compared with ordinary items, there are more attributes that only trigger item $x$ have, which are denoted by $\mathcal{T}_x=[t_x^1, t_x^2, ..., t_x^{N_x^t}]$. $N_t$ denotes the number of all trigger attributes. 
Furthermore, $\mathcal{S}=\{s_1, s_2, ..., s_{N_s}\}$ and $\mathcal{C}=\{c_1, c_2, ..., c_{N_c}\}$ denote the set of $N_s$ scenarios and $N_c$ context features separately. The context features usually describe the page and physical environments of user interaction.
The sequential recommendation is to precisely identify the next item $x_{m+1}$ that user $u$ will click in terms of $\{b_u\}_{M}^N$. 

%============================================
\subsection{Encoder Layer}\label{ssec:encoderlayer}
%============================================
\subsubsection{Embedding Layer} \label{ssec:embeddinglayer}
In the embedding layer, we form six embedding tables:~(1) user embedding table~$U\in R^{N\times d_u}$;~(2) item embedding table~$V\in R^{M\times d_x}$;~(3) attributes embedding table~$A\in R^{(N_a^x+N_a^u)\times d_a}$ including attributes of users and items;~(4) trigger feature embedding table~$T\in R^{{N_t}\times d_t}$;~(5) context feature embedding table~$C\in R^{N_c\times d_c}$;~(6) scenario embedding table~$S\in R^{N_s\times d_s}$, where $d_u$, $d_x$, $d_a$, $d_t$, $d_c$, and $d_s$ denote the representation dimension of the user, item, attribute, trigger, context, and scenario features respectively. For the given target item,  user, attributes, trigger attributes, context, scenario, and the associated behavior sequence, we can perform the table lookup from $U$, $V$, $A$, $T$, $C$, and $S$ to obtain the corresponding embedding representations.

\subsubsection{Query Encoder}
As shown in figure~\ref{sec:intro}, there are two types of queries: (1) Visual query; (2) Trigger query. On one hand, in terms of visual query, we apply the pretrained image embedding in the Alimama platform~\footnote{Here, the image representations can be replaced by other pretrained embeddings or end-to-end training strategy.}, which is denoted by $\mathrm{h}_{img}^q \in R^{512}$. On the other hand, the representation of the trigger item $x$ query is denoted by $\mathrm{h}_x^q = [\mathrm{x}||\mathrm{t}_x^1||\mathrm{t}_x^2||...||\mathrm{t}_x^{N_x^t}]$, where $||$ denotes concatenate operation.

\subsubsection{Sequence Encoder}
According to the section\ref{ssec:embeddinglayer}, we have obtained behavior embedding $[\mathrm{x}_1, \mathrm{x}_2, ..., \mathrm{x}_m]$, and corresponding attributes embedding $[\mathrm{a}_{x_1}, \mathrm{a}_{x_2}, ..., \mathrm{a}_{x_m}]$. Thus, we concatenate the original item representation and its attribute representation, which is shown as follows:
\begin{align}
    \mathrm{h}_x = [\mathrm{x}||\mathrm{a}_x^1||...||\mathrm{a}_x^S].
\end{align}
Finally, the sequence $\mathrm{H}_u$ is represented as follows:
\begin{align}
    \mathrm{H}_u = \{\mathrm{h}_{x_1}, \mathrm{h}_{x_2}, ...\, \mathrm{h}_{x_m}\},
\end{align}
where $m$ denotes the length of each behavior.
Here, we apply Transformer\cite{vaswani2017attention} to capture the interrelation between each item and the whole sequence. 
\begin{align}
    \mathrm{H}_u^{'} = \{\mathrm{h}_{x_1}^{'}, \mathrm{h}_{x_2}^{'}, ...\, \mathrm{h}_{x_m}^{'}\} = Trans(\mathrm{H}_u),
\end{align}
where $Trans$ denotes the transformer operation and the detail can be referred to \cite{vaswani2017attention}. After that, a query-aware attention module is utilized to aggregate the sequence matrix into a vector. Given a query image $\mathrm{h}_{img}^q$ or a query item $\mathrm{h}_x^q$, the following is demonstrated by $\mathrm{h}_{img}^q$.
\begin{align}
    \mathrm{h}_{urb} = \sum_{i=1}^{m} \alpha_i\mathrm{h}_{x_i}^{'}
\end{align}
\begin{align}
    \alpha_i = \frac{exp(sim(\mathrm{h}_{img}^q, \mathrm{h}_{x_i}^{'}))}{\sum_{j=1}^{m}exp(sim(\mathrm{h}_{img}^q, \mathrm{h}_{x_j}^{'}))},
\end{align}
where the $sim$ function denotes the similarity calculation process using Fully Connected(FC) network:
\begin{align}
    sim(x, y) = FC([x||y]).
\end{align}

According to the section~\ref{ssec:encoderlayer}, all features are concatenated as follows:
\begin{align}
    \mathrm{h}_u = [\mathrm{u}||\mathrm{a}_u^1||\mathrm{a}_u^2||...||\mathrm{a}_u^L]
\end{align}
\begin{align}
    \mathrm{h}_{input} = [\mathrm{h}_{urb}||\mathrm{h}_u||\mathrm{h}_{m+1}||\mathrm{h}_{img}^q||\mathrm{h}_{x}^q||\mathrm{h}_c],
\end{align}
where $\mathrm{h}_c$ denotes context embedding.

%============================================
\subsection{Scene-Aware Feature-Grained Scaling}\label{ssec:fgs}
%============================================
Considering the heterogeneity of different scenarios, such as different search modes, it is apparent that features have different influences in different scenarios. For example, visual features generally play a more significant role in photo search than that in scene finding similar items.

Thus, the scene-aware Feature-grained Scaling(FS) module is designed to scale each feature to different degrees according to the scenario indicator, what's more, we also consider the synergistic impact of users' interest and target item. Compared with the previous weight-based approach, the proposed FS calculates the scale alpha $\alpha^{FS}$ ranging from zero to double instead of from zero to one, which is initialized by value one indicating no scaling.
\begin{align}
    \alpha_{FS} = 2*sigmoid(FC([freeze(\mathrm{h}_{input})||\mathrm{u}||\mathrm{x}||\mathrm{h}_s])), \alpha_{FS}\in R^{n}
\end{align}
where $freeze$ denotes the stop gradient operation which aims to avoid the overfitting phenomenon and gradient conflict problem. And there is a double operation in order to enhance the scale operation, where $\alpha_{FS}$ is initialized by ones.
The output of FS module $\mathrm{h}_{FS}$ is calculated as follows:
\begin{align}
    \mathrm{h}_{FS} = [\mathrm{h}_{input}^1 \otimes \alpha_{FS}^1||...||\mathrm{h}_{input}^n \otimes \alpha_{FS}^n],
\end{align}
where $n$ denotes the number of features, $\otimes$ indicates that each feature is multiplied element-wise with corresponding $\alpha_{FS}$.
%============================================
\subsection{Feature-Level Decoupling and Interaction}\label{ssec:fld}
%============================================
Divide the vectors after feature scaling $\mathrm{h}_{FS}$ into different feature domains~(e.g, user domain, query domain, item domain, etc.), which is shown in the bottom part of Figure\ref{fig:model}.
\begin{align}
    \mathrm{h}_{FS} = \{\mathrm{h}_{FS}^1, ..., \mathrm{h}_{FS}^i, ..., \mathrm{h}_{FS}^D\},
\end{align}
where $D$ denotes the number of feature domains, and $\mathrm{h}_{FS}^i$ denotes the representation of $i$-th feature domain.

To mitigate the gradient conflict of feature representation in different scenes, consequently, we design a Feature-Level Decoupling module, which increases the flexibility of fitting multiple scenes with the same feature by adding redundant several Shallow Fully Connected(SFC) layers to each feature domain. In Figure~\ref{fig:model}(a), the number of SFCs is dynamically adjusted according to the coupling degree of the feature domain in multiple scenarios. Further, we hope that scenes with similar data distribution can share SFC, while scenes with gradient conflict can choose other SFCs. The above process is automatically selected by the model during the training process. For this reason, there is a Selecter that takes scene information as input and Gumbel Softmax as the core.
As described, taking an example of the $i$-th feature domain, the mathematical process is described as follows:
\begin{align}
\begin{split}
    \alpha_{SFC}^i = GS(sigmoid(FC([\mathrm{h}_{FS}^i || \mathrm{s}]))), \\ \alpha_{SFC}^i\in R^{N_{SFC}^i},
\end{split}
\end{align}
where $GS$ and $sigmoid$ denote Gumbel Softmax operation and sigmoid activation respectively, and $N_{SFC}^i$ denotes the number of SFCs of the $i$-th feature domain, which is a hyperparameter. Since the Gumbel Softmax discretizes the above selection process, the decoupling ability is further enhanced to some extent. The outputs of the $i$-th feature domain $\mathrm{h}_{SFC}^i$ is defined as follows:
\begin{align}
    \mathrm{h}_{SFC}^i = \alpha_{SFC}^i [FC^1(\mathrm{h}_{FS}^i)||...||FC^{N_{SFC}^i}(\mathrm{h}_{FS}^i)]
\end{align}, 
where $N_{SFC}^i$ denotes the number of SFCs for the $i$-th feature domain. Other domains operate in the same way. 
\begin{align}
    \hat{\mathrm{h}}_{SFC} = [\mathrm{h}_{SFC}^1||...||\mathrm{h}_{SFC}^i||\mathrm{h}_{SFC}^D]
\end{align}.

Nevertheless, this decoupling method also weakens the feature interaction between feature domains obviously, which inspires us to use a Feature Domain Interaction~(FDI) module in Figure~\ref{fig:model}~(a) to enhance cross-domain information explicitly. The specific algorithm refers to pseudo code in algorithm~\ref{algo: FDI}, where $\hat{\mathrm{h}}_{FDI}$ and $\cdot$ denote the interacted output vector and dot product operation respectively.

\begin{algorithm}[]
\caption{Feature Domain Interaction}
\label{algo: FDI}
\LinesNumbered
\KwIn{$\mathrm{h}_{FS} = \{\mathrm{h}_{FS}^1, ..., \mathrm{h}_{FS}^i, ..., \mathrm{h}_{FS}^D\}$}
\KwOut{$\hat{\mathrm{h}}_{FDI}$}
Map the $\mathrm{h}_{FS}^i$ to the same dimension: \
$\widetilde{\mathrm{h}_{FS}} = \{\widetilde{\mathrm{h}_{FS}^1}, ..., \widetilde{\mathrm{h}_{FS}^i}, ..., \widetilde{\mathrm{h}_{FS}^D}\} = \{FC^1(\mathrm{h}_{FS}^1), ..., FC^i(\mathrm{h}_{FS}^i), ..., FC^D(\mathrm{h}_{FS}^D)\}$ \;
Initialize empty list $tmp$ to store the outputs. \


\For{$idx_1$ : 0 -> $size(\widetilde{\mathrm{h}_{FS}})$}{
    \For{$idx_2$ : $(idx_1+1)$ -> $size(\widetilde{\mathrm{h}_{FS}})$}{
    push $(\mathrm{h}_{FS}[idx_1]\cdot \mathrm{h}_{FS}[idx_2])$ into $tmp$ list; 
    }
}
$\hat{\mathrm{h}}_{FDI}$ = Concatenate($tmp$) \;
return $\hat{\mathrm{h}}_{FDI}$; 
\end{algorithm}

Ultimately, the Feature-Level Decoupling and Interaction modules work together to form a more flexible scene-aware shared bottom layer, and we concatenate $\hat{\mathrm{h}}_{SFC}$ and $\hat{\mathrm{h}}_{FDI}$ as the final representation:
\begin{align}
    \hat{\mathrm{h}}_{input} = [\hat{\mathrm{h}}_{SFC}||\hat{\mathrm{h}}_{FDI}].
\end{align}

%============================================
\subsection{Network Layer Decoupling}\label{ssec:nld}
%============================================
In section~\ref{ssec:fgs} and \ref{ssec:fld}, we introduce the feature-level decoupling layer in detail. In this section, we refer to the traditional expert network as the main structure in the network-level decoupling\footnote{Other decoupling solutions of network layers can be replaced according to scenarios and services}. In figure~\ref{fig:model}~(b), experts are selected by Expert Selector through scenario indicator.
\begin{align}
    \mathrm{h}_{NL} = \sum_{j=1}^{N_{e}}g(\mathrm{s})f_j(\hat{\mathrm{h}}_{input}),
\end{align}
\begin{align}
    f_j(x) = \delta(W_jx),
\end{align}
where $N_{e}$ denotes the number of experts in network layer, $\delta(·)$ denotes the relu activation function, and $g(·)$ is gate function which outputs the weights for each experts. 
\begin{align}
    g(x) = softmax(W_gx),
\end{align}
where $W_g$ and $W_j$ are learnable parameters.

%============================================
\subsection{Prediction and Model Optimization}\label{ssec:predictor}
%============================================
\subsubsection{Prediction}
In prediction-level layer, we draw lessons from the advantages of multi-tower structure, and use independent prediction towers for each scenario in the prediction phase, namely $FCN^{i}(·)$. In addition, an extra tower is used to provide shared information from other scenes, among which the most important is to calculate the weights based on the average similarity between the current scene and other scenes. 
\begin{align}
    \mathrm{h}_{sp}^s = FCN^{s}(\mathrm{h}_{NL}),
\end{align}
where $\mathrm{h}_{sp}^s$ denotes the specific representation for $s$-th scene.
\begin{align}
    \mathrm{h}_{sh}^s = \alpha_{sh}^sFCN_{sh}(\mathrm{h}_{NL}),
\end{align}
\begin{align}
    \alpha_{sh}^s = \frac{1}{N_s}\sum_{i=1}^{N_s}\mathrm{h}_{s}\mathrm{h}_{s}^i,
\end{align}
where $\mathrm{h}_{sh}^s$ denotes the shared representation from extra tower $FCN_{sh}(·)$ for current scene, and $\alpha_{sh}^s$ denotes the weights of the outputs of extra tower for current scene.
Ultimately, the prediction vector is calculated as follows:
\begin{align}
    \mathrm{h}_{p} = \mathrm{h}_{sp}^s + \mathrm{h}_{sh}^s.
\end{align}

\begin{align}
\hat{y} = FCN(\mathrm{h}_{p}),
\label{eq:score}
\end{align}
where $\hat{y}$ denotes the prediction score for user, query, and target triple. 

\subsubsection{Model Optimization}
For the sake of ensuring the high mobility, universality and efficiency of the model, all samples use the same optimization method, although there are multiple scenarios in the dataset. Thus, the final loss is formulated as follows:
\begin{align}
    \label{eq:finalloss}
    \mathcal{L}_{final} &= \mathcal{L}_1 + \theta\mathcal{L}_2, \\
    \mathcal{L}_1 &= -\sum_{u,i}[yln(\hat{y}) + (1-y)ln(1-\hat{y})],
\end{align}
where $y$ denotes the ground truth, $\mathcal{L}_2$ denotes the $L_2$ norm of all model parameters,  $\theta$ denote the hyperparameters.





==> intro_backup.tex <==
\section{Introduction}\label{sec:intro}
\begin{figure}[!]
    \centering
    \includegraphics[width=\linewidth]{img_new/figure_intro1.pdf}
    \caption{Two representative channels in the left side consists of three different scenarios with different search modes in the middle of the figure. And result contexts corresponding to each scenario are shown in the right side.}
    \label{fig:intro1}
\end{figure}
With the rapid development of the Internet, it is usually that users' behavior covers multiple scenes, in other words, the business of a company is diversified and complicated. 
In this situation, the division of scenes is probably according to the different user groups, such as new and old users, and different sub-channel of mobile applications. Instead, diverse client media can also be viewed as multiple scenarios.
For instance, Figure~\ref{fig:intro1} shows two representative business channels in Alimama including three main retrieval scenarios except text retrieval.  
\begin{itemize}
    \item Visual Query Scenario: In addition to text search, users can use their mobile phones to take photos for image search.
    \item Item Query Scenario: The user searches the retrieved items for a second time, that is, to find similar items. The user's intention of secondary retrieval is relatively complex, and there may be such intentions as price comparison and searching for items in the same style.
    \item Advertisements~(Ads) Query Scenario: The channel of this scenario is different from that of the above scenarios. It is the external media. When users click on an external media advertisement, they jump to the mobile Taobao page and the search results on the current page are displayed.
\end{itemize}
Considering the form and content of the page presentation and the various intents of users, the data distribution in different scenarios has significant deviation. More specifically, for example, in figure~\ref{fig:intro1}, result contexts from different scenarios have different page environments and feedback results, among which the user's intentions and concerns are also quite different.

Traditional models~\cite{cheng2016wide, guo2017deepfm, koren2009matrix, rendle2010factorization, schafer2007collaborative, sarwar2001item, zhou2019deep, zhang2016deep, zhou2018deep, shan2016deep, tian2022multi} serve each scenario with their own data, and the number of models corresponds to the number of scenarios. However, there are two defects that become more and more worrisome with the development:~(1) some scenarios have a small amount of data and models do not converge effectively;~(2) It takes too many resources to train and inference alone, and it is troublesome to upgrade and maintain in the future. Hence, Multi-Scenario Learning~(MSL) emerges as the times require.

In an effort to improve the performance of MSL, the scientists focus on how to model the commonness and differences between scenes at the same time. In general, all methods can be summarized into three paradigms: Auxiliary Paradigm,  Expert Paradigm, and Multi-Tower Paradigm, which are shown in figure~\ref{fourParadigm}~(a, b, c). In the terms of the structures of these solutions, inputs from all scenes share the same embedding bottom but differ greatly in the network layer obviously. The decoupling method of the network layer has been proven to have a very positive performance, but now the rigid shared bottom structure has become the bottleneck currently, especially when there is a big difference between the scenes, such as that shown in Figure~\ref{fig:intro1}.

\begin{figure*}[!]
  \centering
  \begin{subfigure}{0.24\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{img_new/paradigms_1.pdf}
		\caption{Auxiliary Paradigm}
		\label{paradigm1}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{img_new/paradigms_2.pdf}
		\caption{Multi-tower Paradigm}
		\label{paradigm2}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{img_new/paradigms_3.pdf}
		\caption{Expert Paradigm}
		\label{paradigm3}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
		\centering
		\includegraphics[width=0.9\linewidth]{img_new/paradigms_4.pdf}
		\caption{Ours}
		\label{paradigm4}
  \end{subfigure}
  \caption{Classical paradigms structure and ours.}
  \label{fourParadigm}
\end{figure*}

To this end, in this paper, we propose a new paradigm: scene-aware \textbf{F}e\textbf{A}ture-level \textbf{D}ecoupling and \textbf{IN}teraction modelin\textbf{G} approach~(named \baby). Specifically, \baby is developed with a multi-level decoupling structure covering feature level, network level, and prediction level. We propose an agile scene-aware shared bottom that subverts the traditional multi-scenario learning paradigm including two main components: \textit{Feature-Grained Scaling} and \textit{Feature-Level Decoupling and Interaction}. The comparison between traditional solutions and ours is shown in figure~\ref{fourParadigm}. We introduce multiple independent mapping matrices for each feature domain and learnable processes to guide each scene to select different mapping matrices to fine-tune the bottom representation. In this way, the traditional rigid shared bottom structure is replaced by a self-adjustable scene-aware manner. Afterwards, we perform an explicit interaction for every two feature domains in order to supplement the cooperation information between various feature domains.
To summarize, the contributions of this paper are as follows:

\begin{itemize}
    \item We propose a novel multi-scenario learning paradigm, which not only focuses on the network layer but also proposes a multi-level decoupling and sharing structure including feature level, network level, and prediction level respectively.

    \item We devise a scene-aware shared bottom improving the flexibility of shared representation without increasing the consumption of parameter amounts explicitly. More specifically, we utilize Feature-Grained Scaling to distinguish the more influential features. Further, a Feature-Level Decoupling and Interaction module guides each scene to fine-tune the scene-aware representation effectively.
    
    \item We conduct extensive experiments on two large-scale datasets collected from real-world applications. The experimental results show significant performance improvements compared with the state-of-the-art technique alternatives. Further analysis and experiments are provided to demonstrate the effectiveness and practicability of \baby.
\end{itemize}
